Throughput of Freeway Networks under Ramp Metering Subject to Vehicle Safety Constraints

Ramp metering is one of the most effective tools to combat traffic congestion. In this paper, we present a ramp metering policy for a network of freeways with arbitrary number of on- and off-ramps, merge, and diverge junctions. The proposed policy is designed at the microscopic level and takes into account vehicle following safety constraints. In addition, each on-ramp operates in cycles during which it releases vehicles as long as the number of releases does not exceed its queue size at the start of the cycle. Moreover, each on-ramp dynamically adjusts its release rate based on the traffic condition. To evaluate the performance of the policy, we analyze its throughput, which is characterized by the set of arrival rates for which the queue sizes at all on-ramps remain bounded in expectation. We show that the proposed policy is able to maximize the throughput if the merging speed at all the on-ramps is equal to the free flow speed and the network has no merge junction. We provide simulations to illustrate the performance of our policy and compare it with a well-known policy from the literature.

==> arXiv_Adaptive.tex <==
\section{Adaptive FCQ Ramp Metering policy}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Definition %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}\label{Def: Fixed-Cycle Quota RM policy}
\textbf{(Fixed-Cycle Quota Ramp Metering (FCQ-RM) policy)} The policy works in cycles of fixed length $\Cyclelength \in \N$. At the beginning of the $k^{th}$ cycle at $t_k = (k-1)\Cyclelength$, for all $k \geq 1$, each on-ramp allocates itself a ``quota" equal to the queue length at that on-ramp at $t_k$. During the cycle $t \in [t_k, t_{k+1}]$, each on-ramp releases a vehicle whenever a safe virtual slot appears, until it reaches its quota. Once an on-ramp reaches its quota, it does not release a vehicle during the rest of the cycle. 
\end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Definition %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Remark %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{remark}\label{Rem: eps-unsafe FCQ-RM}
One should note that the proposed FCQ-RM policies are fragile to arbitrarily small perturbations in vehicle locations. This is mainly due to strict safety criteria. In order to make up for possible inefficiencies, one can adopt $\eps$-unsafe FCQ-RM policies which allow merging if the slot is within $\eps$ distance of safe position. 
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Remark %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Definition %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}\label{Def: Distributed Adaptive FCQ-RM}
\textbf{(Adaptive FCQ-RM (aFCQ-RM) policy)} 
The policy works in cycles of fixed length $\Cyclelength \in \N$. At the beginning of the $k^{th}$ cycle at $t_k = (k-1)\Cyclelength$, for all $k \geq 1$, each on-ramp allocates itself a "quota" equal to the queue length at that on-ramp at $t_k$. During the cycle $t \in [t_k, t_{k+1}]$, the $j^{th}$ on-ramp releases a vehicle if a safe virtual slot appears, and at least $\Releasetime{j}(t)$ time has passed since the release of the last vehicle. Once an on-ramp reaches its quota, it does not release a vehicle during the rest of the cycle. The minimum time gap $T_j(t)$ for on-ramp $j$ is piecewise constant, updated periodically at $t = \updateperiod, 2\updateperiod, \ldots$ according to algorithm \ref{Alg: aFCQ-RM policy}.
\begin{algorithm}[H]
\caption{Update rule for the minimum time gap between release of vehicles under the caFCQ-RM policy}\label{Alg: aFCQ-RM policy}
\begin{algorithmic}
\Require $\updateperiod>0,\DesDecreaseconst{} > 0$, $\theta_1 > 0$, $\theta^{0}_{2} > 0$, $\beta > 1$, $(\Releasetime{j}(0), \theta_2(0)) = (0, \theta^{0}_{2}), j \in [\numramps]$

\hspace{-0.475in} \textbf{for} $t = \updateperiod, 2\updateperiod, \cdots$ \textbf{do} the following for each on-ramp $j \in [\numramps]$
\If{$\Releasetime{j+1}(t-1) \leq T_{max}$}
\If{$\|\StateofDySys_{j}(t)\| \leq \max\{\|\StateofDySys_{j}(t-1)\| - \DesDecreaseconst{}, 0\}$ } 
\State $\Releasetime{j}(t) \gets \max\{\Releasetime{j}(t-1) - \theta_1, 0\}$
\Else{}
\If{$\|\StateofDySys_{j}(t-1)\| \leq \max\{\|\StateofDySys_{j}(t-2)\| - \DesDecreaseconst{}, 0\}$}
\State $\theta_2(t) \gets \beta \theta_2(t-1)$
\State $\Releasetime{j}(t) \gets \Releasetime{j}(t-1) + \theta_2(t)$
\Else{}
\State $\theta_2(t) \gets \theta_2(t-1)$
\State $\Releasetime{j}(t) \gets \Releasetime{j}(t-1) + \theta_2(t-1)$
\EndIf
\EndIf
    \Else{}
\State $\theta_2(t) \gets \theta_2(t-1)$
\State $\Releasetime{j}(t) \gets \Releasetime{j}(t-1) + \theta_2(t)$
\EndIf

\hspace{-0.475in} \textbf{end for}
\end{algorithmic}
\end{algorithm}
\end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Definition %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% Proposition %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{Prop: stability of aFCQ-RM}
Let the merging speed at all of the on-ramps be $\speedlim$. For any cycle length $\Cyclelength$ and design constants $\updateperiod, \DesDecreaseconst{}, \ReleasetimeDec, \ReleasetimeInc^{0} > 0$, $\ReleasetimeAdj{} > 1$, the aFCQ-RM policy keeps the network under-saturated if and only if $\Avgload{} < 1$.
\end{proposition} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% Proposition %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
It is sufficient to show that $\|\StateofDySys(k\updateperiod)\| = 0$ for some positive integer $k$. This would then imply that $\Releasetime{}(\cdot) = 0$ after a finite time. Thereafter, the aFCQ-RM policy coincides with the FCQ-RM policy, and therefore, the result follows from Theorem \ref{Prop: Stability of FCQ-RM policy for all T}.  
\par
We use a proof by contradiction. Suppose that for all $k \in \Z_{+}$, $\|\StateofDySys(k\updateperiod)\| \neq 0$. Thus, there exists a link $j \in [\numramps]$ such that $\|\StateofDySys_j(k\updateperiod)\| \neq 0$ for infinitely many $k$'s. We claim that this would imply $\limsup_{k \ra \infty} \Releasetime{j}(k \updateperiod) = \infty$. To show this, we note that if 
\begin{equation*}
    \|\StateofDySys_{j}(t)\| \leq \max\{\|\StateofDySys_{j}(t-1)\| - \DesDecreaseconst{}, 0\}
\end{equation*}
for $t = k\updateperiod$ at finitely many $k$'s, then by the description of Algorithm \ref{Alg: aFCQ-RM policy} we must have $\limsup_{k \ra \infty}\Releasetime{j}(k \updateperiod) = \infty$. Otherwise, since $\|\StateofDySys_j(\cdot)\| \leq \|\StateofDySys(\cdot)\|$ is (uniformly) bounded, there exists infinitely many $k$'s such that at $t = k \updateperiod$ we have
\begin{equation*}
    \begin{aligned}
        \|\StateofDySys_{j}(t)\| &> \max\{\|\StateofDySys_{j}(t-1)\| - \DesDecreaseconst{}, 0\}, \\
        \|\StateofDySys_{j}(t-1)\| &\leq \max\{\|\StateofDySys_{j}(t-2)\| - \DesDecreaseconst{}, 0\}.
    \end{aligned}
\end{equation*}
\par
Since $\ReleasetimeInc(t)$ is non-decreasing with jumps of size $\beta$ whenever occurs, it follows that $\limsup_{k \ra \infty}\ReleasetimeInc(k\updateperiod) = \infty$. As a result, $\limsup_{k \ra \infty}\Releasetime{j}(k \updateperiod) = \infty$. Let $\hat{k}$ be such that
\begin{equation*}
    \Releasetime{j}(\hat{k}\updateperiod) > \left(1 + (\numramps - 1)\frac{\ReleasetimeDec}{\ReleasetimeInc^{0}}\right)\max\{T_{max}, (\numramps + 1)\Tempty\}.
\end{equation*}
\par
The description of Algorithm \ref{Alg: aFCQ-RM policy} then implies that at time $t = (\hat{k} + (\numramps - 1)\lceil \frac{\ReleasetimeDec}{\ReleasetimeInc^{0}} \rceil)\updateperiod$ we must have 
\begin{equation*}
    \Releasetime{i}(t) \geq \max\{T_{max}, (\numramps + 1)\Tempty\},
\end{equation*}
for all $i \in [\numramps]$. Hence, no on-ramp releases a vehicle for at least $(\numramps + 1)\Tempty$ time units after the last time they released one at or before $t$. Thus, there exists a time interval of length $\Tempty$ in $[t, t + (\numramps + 1)\Tempty]$ during which no on-ramp releases a vehicle. Assumption~\ref{Assum: Vehicles accelerate when they find safe gap} then implies that the ring road is empty after such $\Tempty$ time units, at the end of which $\|X(\cdot)\|=0$; a contradiction. Therefore, there exists $k \in \Z_{+}$ such that $\|\StateofDySys(k\updateperiod)\| = 0$. 
\end{proof}

==> arXiv_Example.tex <==
\section{Examples}\label{sec:example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Figure %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/ThreeLeggedNtwrk.png}
    
    \vspace{0.2 cm}
    
    \caption{\sf A three-legged merge network, with $\numsources = 6$ \source{s} and $\numsinks = 4$ \sink{s}}
    \label{fig: Three-legged merge network}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Figure %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Consider a three-legged merge junction, where two freeway links enter, and a single freeway link leaves the merging point; see Figure~ . There are a total of $\numsources$ \emph{\source{s}}, to which \agent{s} arrive, and $\numsinks$ \emph{\sink{s}}, from which \agent{s} leave the network. The \source{s} and the \sink{s} are spread across all three links. Let the \agent{s} arrive to source $i \in [\numsources]$ according to an i.i.d Bernoulli process with parameter $\Arrivalrate{i} \in [0,1]$. These processes are independent across different \source{s}. That is, in any given time step, the probability that an \agent{} arrives at the $i$-th \source{} is $\Arrivalrate{i}$ independent of everything else. The intended \emph{\pas{}} for individual arriving \agent{s} is i.i.d. and is given by a \textit{routing matrix} $\routingmatrix = [\routingmatrix_{ip}]$, where $0 \leq \routingmatrix_{ip} \leq 1$ is the probability that an arrival to \source{} $i$ wants to use \pas{} $p$ in order to exit from some \sink{} $j \in [\numsinks]$. Note that in the current three-legged network, a $\pas{}$ is uniquely determined by its starting \source{} and ending \sink{}.
\par
To conveniently track vehicle locations in discrete time, we introduce the notion of \emph{slot}. A slot is associated with a particular point on one of the links at a particular time. Let $\numcells{i}$ be the maximum number of distinct points that can be placed on the $i$-th link, $i \in [3]$, such that the distance between adjacent points is $\timeheadway \speedlim + \standstilldist + \vehiclelength$, i.e., the safety distance at the free flow speed. Consider a configuration of the slots at $t = 0$. Note that, within each link, each slot replaces the next slot at the end of each time step $\timestep$. Without loss of generality, we assume that the configuration of slots on different links are such that, for every junction, the last slot of every incoming link replaces the first slot of every outgoing link.   
\par
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Figure %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb!]
\begin{center}
    \begin{subfigure}{.437\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/MergeEx_optimal.png}
        \caption{} \label{fig:optimal-merge-example}
    \end{subfigure}
    \begin{subfigure}{.45\textwidth}
    \vspace{0.3 cm}
        \centering
        \includegraphics[width=\textwidth]{Figures/MergeEx_suboptimal.png}
        \caption{} \label{fig:suboptimal-merge-example}
    \end{subfigure}
    \end{center}
    \vspace{0.2 cm}
    \caption{\sf A network with $3$ \source{s}, $1$ \sink{}, a merge, and a diverge junction.}
    \label{fig:merge-example}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Figure %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% Example %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{example}
Consider the network of Figure~\ref{fig:merge-example} under the following ramp metering policy: \source{} $1$ uses every slot to release an \agent{}, \source{s} $2$ and $3$ use every other nonconflicting slots to release \agent{s}. Let the arrival process at \source{s} $1$ and $2$ be given by $\Numarrivals{1}(k\timestep)=1$, and $\Numarrivals{2}(2k\timestep)=1$ for all $k \in \N$.  Consider the following two cases: in the first case, an \agent{} arriving to \source{} $1$ at time $k\timestep$ takes the upper link at the diverge junction if $k$ is odd; otherwise, it takes the lower link. In the second case, it takes the upper link if $k = 4k'+1, 4k'+2$ for some $k' \in \N$; otherwise, it takes the lower link. Notice that the arrival rate and the routing matrix are the same in both cases. However, the network remains undersaturated in the first case, while it becomes saturated in the second case.
\end{example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% Example %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> arXiv_Notations.tex <==
\section{Notations}

\begin{center}
\begin{tabular}{ll} 
$\numsources$: & set of sources
\\
$\numsinks$: & number of sinks
\\
node, \route: & a vector of nodes

\end{tabular}
\end{center}

We collect key notations to be used throughout the paper. Let $\N$ and $\R$ respectively denote the set of natural and real numbers. For $m \in \N$, $[m]$ denotes the set $\{1, \ldots, m\}$.

==> proof-sketch-ACC.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% Appendix %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof Sketch for Theorem \ref{Prop: stability of DRR-RM}}\label{sec:proof-sketch}
For any initial condition, we can show that there exists some $k_0 \in \N$ such that for all $k \geq k_0$, $\StateofDySys_f(k\updateperiod) = 0$. This and (VC1) imply that every \agent{} moves at the free flow speed for all $t \geq t_0$. Hence, after a finite time after $t_0$, $\Releasetime{}(\cdot)=0$, and the location of every \agent{} coincides with a slot thereafter. 
\par
Consider now an initial condition where the \agent{s} are in the free flow equilibrium, and the location of each \agent{} coincides with a slot. Thus, their location coincide with a slot in the future. Thereafter, during each time step, the following sequence of events occurs: (i) the slots on each segment replace the next slot with the last slot replacing the first slot; the numbering of slots is reset with the new first slot numbered $1$, and the rest numbered in an increasing order in the direction of the flow, (ii) \agent{s} that reach their destination \sink{} exit the network, (iii) if permitted by the ramp metering policy, a \agent{} is released into a slot at the free flow speed. Since the initial location of all \agent{s} coincide with a slot and the released times are conflict-free, the location of the released \agent{} will also coincide with a slot in the future.
\par
For the aforementioned initial condition, we can cast the network as a discrete-time Markov chain, with time steps of size $\timestep$. Let $M(n)$ be the set of the \route{s} of the occupants of all the slots: $M_{\ell}(n)=p$ if the \agent{} occupying slot $\ell$ at time $n$ has to take route $p$, and $M_{\ell}(n)=0$ if slot $\ell$ is empty at time $n$. 
%We use $|M(n)|$ to denote the number of \agent{s} on the mainline at time $n$. 
Consider the following discrete-time Markov chain with the state 
%\begin{equation*}
    $\StateofMCExp_{\triangle}(n) := \StateofMC(n\triangle)$, $n \geq 0$,
%\end{equation*}
where $\StateofMC(n) := (\Queuelength{}(n),\Nodedest{}(n))$, and $\triangle \in \N$ is a constant that will be determined in the course of the proof. For the $\DRR$ policy, the state $\StateofMC(n) = (0, 0)$ is reachable from all the other states, and $\mathbb{P}\left(\StateofMC(n+1) = (0, 0)~|~ \StateofMC(n) = (0,0)\right) > 0$. Hence, the Markov chain $\StateofMCExp_{\triangle}$ is irreducible and aperiodic. 
\par
Finally, we can find a Lyapunov function $V: \StateSpace \ra [0,\infty)$ that satisfies
\begin{equation*}
\begin{aligned}
    \mathbb{E}\left[\Lyap{n+1} - \Lyap{n}|\: \StateofMCExp_{\triangle}(n)\right] \leq -\|\Queuelength{}(n\triangle)\|_{\infty} + b\mathds{1}_{B},
\end{aligned}
\end{equation*} 
where $\StateSpace$ is the range of $Y$, $b$ is a constant, $B$ is a finite set, and $\|\Queuelength{}(n\triangle)\|_{\infty} = \max_{i \in \numsources}|\Queuelength{i}(n\triangle)|$. The result then follows from the well-known Foster-Lyapunov drift criterion \cite[Theorem 14.0.1]{meyn2012markov}.
